On the shape of the general error locator polynomial for cyclic codes

A general result on the explicit form of the general error locator polynomial for all cyclic codes is given, along with several results for infinite classes of cyclic codes with $t=2$ and $t=3$. From these, a theoretically justification of the sparsity of the general error locator polynomial is obtained for all cyclic codes with $t\leq 3$ and $n<63$, except for three cases where the sparsity is proved by a computer check. Moreover, we discuss some consequences of our results to the understanding of the complexity of bounded-distance decoding of cyclic codes.

==> symbols.tex <==
\usepackage{amssymb,amsmath,amsthm,xcolor,stmaryrd}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsthm}
\usepackage{latexsym}
\usepackage{hyperref}  
\usepackage{anysize}

\usepackage{enumerate}

\usepackage{url,times,verbatim,multirow,tikz}
\usetikzlibrary{matrix}
%%% 
%%% format style
%%%
%%% 
%%% format style
%%%
\setlength{\topmargin}{0pt}
\setlength{\textheight}{9in}
\setlength{\headheight}{0pt}
\setlength{\headsep}{0pt}
\setlength{\oddsidemargin}{0.25in}
\setlength{\textwidth}{6in}
\setlength{\parindent}{1pc} % set indent to null
\setlength{\parskip}{3pt}

\pagestyle{plain}



%%%
%%% comments
%%%
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\commentM}[1]{\textcolor{red}{{\sf (Manuela's Note:)} {\sl{#1}}}}
\newcommand{\commentC}[1]{\textcolor{green}{{\sf (Claudia's Note:)} {\sl{#1}}}}
\newcommand{\commentMax}[1]{\textcolor{blue}{{\sf (Max's Note:)} {\sl{#1}}}}

%%%
%%% notation
%%%


\newenvironment{rostera}
{\begin{enumerate}[\upshape(a)]}
{\end{enumerate}}

\newcommand{\vc}{\mathbf{c}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vs}{\mathbf{s}}

\newcommand{\bp}{\mathsf{h}}
\newcommand{\wbp}{\mathsf{wh}}
\newcommand{\gelp}{\mathsf{gelp}}


\newcommand{\F}{\mathbb{F}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\ZZ}{{\mathbb Z}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\CC}{{\mathbb C}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\KK}{{\mathbb K}}
\newcommand{\GR}{Gr\"{o}bner}
\newcommand{\Gr}{Gr\"{o}bner}
\newcommand{\Special}{s2ec code}
\newcommand{\spl}{s2ec}
\newcommand{\splint}{s2ec--integer}
%\newcommand{\ns}{\mathrm{ns}}
%\newcommand{\spp}{\mathrm{sp}}
%\newcommand{\spd}{\mathrm{spd}}
%\newcommand{\SPD}{\mathrm{SPD}}
%\newcommand{\spz}{\mathrm{spz}}
\newcommand{\spnz}{\mathrm{spnz}}
\newcommand{\Cyc}{\mathrm{Cyclic}}
\newcommand{\JC}{\tilde J_C}
\newcommand{\lp}{\mathrm{Lp}}
\newcommand{\tp}{\mathrm{Tp}}

\newcommand{\fattorial}[2]{ \left( #1 \atop #2 \right) }
\newcommand{\h}{\hspace{0.4cm}}
\newcommand{\hi}{\hspace{0.2cm}}

\newfont{\gotico}{eufm10 scaled \magstep1}


%%%
%%% theorems, definitions etc
%%%
%% roba da Mora

\def\card{\mathop{\rm card}\nolimits}
\def\mappa#1{\smash{\mathop{\longrightarrow}\limits^{#1}}}
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\quad
\ifmmode\squareforqed\else{\squareforqed \medskip}\fi}
\def\then{\Longrightarrow}
\def\text#1{\rm #1}
\def\emph#1{\em #1}
\def\Lou{Loustaunau}
%\def\lc{\mathop{\rm lc}\nolimits}
\def\chart{\mathop{\rm char}\nolimits}
%\newcommand{\Gr}{Gr\"ob\-ner}

%\renewcommand\thetheorem{\arabic{section}.\arabic{theorem}}
\newtheorem{theorem}{Theorem} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{lemmabis}[theorem]{Remark and Notation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{History}[theorem]{Historical Remark}
\newtheorem{Fact}[theorem]{Fact}
%\newtheorem{lemmavoid}[]{}

% con i seguenti comandi puoi scegliere di mettere un quadratino alla fine degli esempi
% e rendere il testo dunque piu' leggibile
\newtheorem{ex*}[theorem]{Example}
\newtheorem{exas*}[theorem]{Examples}
\newenvironment{ex}{\begin{ex*}}{\qed\end{ex*}}
\newenvironment{exas}{\begin{exas*}}{\qed\end{exas*}}

%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
% con i seguenti comandi puoi scegliere di mettere un quadratino alla fine degli esempi
% e rendere il testo dunque piu' leggibile


\def\Cal#1{{\cal #1}}

%%%
%%% figures
%%%
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figlab}[1]{\label{fig:#1}}
\newenvironment{boxfig}[2]{% {#1}{#2} = {Caption}{label}
     \begin{figure}[htb!]
     \newcommand{\FigCaption}{#1}
     \newcommand{\FigLabel}{#2}
       \vspace{-0.60cm}
     \begin{center}
       \begin{small}
         \begin{tabular}{@{}|@{~~}l@{~~}|@{}}
           \hline
           \rule[-1.5ex]{0pt}{1ex}\begin{minipage}[b]{.96\linewidth}
             \vspace{1ex}
             \smallskip
             }{%
           \end{minipage}\\
           \hline
         \end{tabular}
       \end{small}
       \vspace{-0.2cm}
       \caption{\FigCaption}
       \figlab{\FigLabel}
     \end{center}
     \vspace{0.2cm}
   \end{figure}
}


\usepackage{fullpage}
\usepackage{array}
\newenvironment{custommargins}[2]%
  {\addtolength{\leftskip}{#1}\addtolength{\rightskip}{#2}}{\par}

